Chiral and directional optical emission from a dipole source coupled to a helical plasmonic antenna

Plasmonic antennas with helical geometry are capable transducers between linearly polarized dipole emission and purely circular polarized far-fields. Besides large Purcell enhancements they possess a wide tunability due to the geometry dependence of their resonant modes. Here, the coupling of a dipole emitter embedded in a thin film to plasmonic single and double helices is numerically studied. Using a higher-order finite element method (FEM) the wavelength dependent Purcell enhancement of a dipole with different positions and orientations is calculated and the far-fields with respect to their chirality and radiation patterns are analyzed. Both single and double helices demonstrate highly directional and circularly polarized far-fields for resonant excitation but with significantly improved directional radiation for the case of double helices.

==> Bilder/Single_Helix_Feldbilder_1103nm.tex <==
\begin{tikzpicture}
   % Erste Mode - Single Helix
   \draw ( 0,0) node{\includegraphics[scale=0.16]{Bilder/Single_Helix_Lambda_1103nm_legende.png}};
   \draw (-0.9,1.4) node{1e+32};
   \draw (-0.9,2.3) node{2e+35};

%   % Zweite Mode - Single Helix
%   \draw ( 4.5,0) node{\includegraphics[scale=0.2]{Bilder/Single_Helix_Lambda_1276nm _legende.png}};
%   \draw (3.3,1.7) node{1e+32};
%   \draw (3.3,3) node{2e+35};

%   % Dritte Mode - Single Helix
%   \draw ( 9,0) node{\includegraphics[scale=0.2]{Bilder/Single_Helix_Lambda_1606nm_legende.png}};
%   \draw (7.8,1.7) node{1e+32};
%   \draw (7.8,3) node{2e+35};
   
\end{tikzpicture}

==> Bilder/Single_Helix_Feldbilder_1276nm.tex <==
\begin{tikzpicture}
%   % Erste Mode - Single Helix
%   \draw ( 0,0) node{\includegraphics[scale=0.2]{Bilder/Single_Helix_Lambda_1103nm_legende.png}};
%   \draw (-1.2,1.7) node{1e+32};
%   \draw (-1.2,3) node{2e+35};

   % Zweite Mode - Single Helix
   \draw ( 0,0) node{\includegraphics[scale=0.16]{Bilder/Single_Helix_Lambda_1276nm _legende.png}};
   \draw (-0.9,1.4) node{1e+32};
   \draw (-0.9,2.3) node{3e+35};

%   % Dritte Mode - Single Helix
%   \draw ( 9,0) node{\includegraphics[scale=0.2]{Bilder/Single_Helix_Lambda_1606nm_legende.png}};
%   \draw (7.8,1.7) node{1e+32};
%   \draw (7.8,3) node{2e+35};
   
\end{tikzpicture}

==> Bilder/Single_Helix_Feldbilder_1606nm.tex <==
\begin{tikzpicture}
%   % Erste Mode - Single Helix
%   \draw ( 0,0) node{\includegraphics[scale=0.2]{Bilder/Single_Helix_Lambda_1103nm_legende.png}};
%   \draw (-1.2,1.7) node{1e+32};
%   \draw (-1.2,3) node{2e+35};

%   % Zweite Mode - Single Helix
%   \draw ( 4.5,0) node{\includegraphics[scale=0.2]{Bilder/Single_Helix_Lambda_1276nm _legende.png}};
%   \draw (3.3,1.7) node{1e+32};
%   \draw (3.3,3) node{2e+35};

   % Dritte Mode - Single Helix
   \draw ( 0,0) node{\includegraphics[scale=0.16]{Bilder/Single_Helix_Lambda_1606nm_legende.png}};
   \draw (-0.9,1.4) node{1e+32};
   \draw (-0.9,2.3) node{3e+35};
   
\end{tikzpicture}
